Gradient-based optimisation of the conditional-value-at-risk using the multi-level Monte Carlo method

In this work, we tackle the problem of minimising the Conditional-Value-at-Risk (CVaR) of output quantities of complex differential models with random input data, using gradient-based approaches in combination with the Multi-Level Monte Carlo (MLMC) method. In particular, we consider the framework of multi-level Monte Carlo for parametric expectations and propose modifications of the MLMC estimator, error estimation procedure, and adaptive MLMC parameter selection to ensure the estimation of the CVaR and sensitivities for a given design with a prescribed accuracy. We then propose combining the MLMC framework with an alternating inexact minimisation-gradient descent algorithm, for which we prove exponential convergence in the optimisation iterations under the assumptions of strong convexity and Lipschitz continuity of the gradient of the objective function. We demonstrate the performance of our approach on two numerical examples of practical relevance, which evidence the same optimal asymptotic cost-tolerance behaviour as standard MLMC methods for fixed design computations of output expectations.

==> sections/new_content.tex <==
{\color{red}
We now wish to study the performance of the \gls{amgd} algorithm for different significances $\tau$.
To this end, we compare the performance of the algorithm for $\tau=0.7$ and $\tau=0.9$.
Since the performance of the algorithm in terms of objective function and gradient decay in the $\tau=0.9$ case are nearly identical to the performance observed in Fig.~\ref{fig:pol_comp_performance} for the $\tau=0.7$, the corresponding results are not presented here.
Fig.~\ref{fig:pol_hierarchy_sig} shows the optimal hierarchy produced by the \gls{cmlmc} algorithm at each optimisation iteration for the two significances tested.
We observe that the level-wise sample sizes $N_l$ decay at the same rate in the levels $l$ for both tested significances, however with a larger constant for the $\tau=0.9$ case.
Additionally, Fig.~\ref{fig:pol_opti_complexity_sig} shows the cumulative cost for a given gradient magnitude, for both significances.
We observe that the cumulative cost grows as $\norm{\objestgrad(w_j)}_{\sltwo}^{-2}$ in both cases, following an initial pre-asymptotic regime.
However, the $\tau=0.9$ case shows a larger constant.
In this case, the interval $\Theta$ is changed with each optimisation iteration such that it is centered on the quantile estimate corresponding to the previous optimisation iteration.
It can be shown, for the case of a simple Monte Carlo estimator, that the constant is expected to scale in this case as $(1-\tau)^{-1}$.
We note that we observe a similar scaling in this case.
}
\begin{figure}[h]
  \centering
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{img/optimization_samples_pol_sig}
    \caption{Level-wise sample sizes}
    \label{fig:pol_hierarchy_sig}
  \end{subfigure}
  \begin{subfigure}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{img/optimization_complexity_pol_sig}
    \caption{Cumulative cost}
    \label{fig:pol_opti_complexity_sig}
  \end{subfigure}
  \caption{Hierarchy and complexity behaviour for different significances for pollutant transport problem}
  \label{fig:pol_comp_performance_sig}
\end{figure}

{\color{red}
\paragraph{Remark 3.} We remark that $\eta$ is a monotonically increasing function of the product $\alpha \mu$ in the interval $0 < \alpha \mu \leq 1$.
For an appropriate step size $\alpha$, chosen such that $\alpha \mu$ is close to $1$, $\eta$ can be as large as $~0.4$.}


